RustMap: Towards Project-Scale C-to-Rust Migration via Program Analysis and LLM

Migrating existing C programs into Rust is increasingly desired, as Rust offers superior memory safety while maintaining C's high performance. However, vastly different features between C and Rust--e.g., distinct definitions and usages of pointers and references--pose significant challenges beyond mere syntactic translation. Existing automated translation tools, such as C2Rust, may rely too much on syntactic, template-based translation and generate unsafe Rust code that is hard for human developers to read, maintain, or even compile. More semantic-aware translation that produces safer, idiomatic, and runnable Rust code is much needed. This paper introduces a novel dependency-guided and large language model (LLM)-based C-to-Rust translation approach, RustMap, based on three key ideas: (1) Utilize LLM capabilities to produce idiomatic Rust code from given small pieces of C code, (2) Mitigate LLM limitations in handling large codebases by breaking project-scale C programs into smaller units for translation according to their usage dependencies and composing them into a runnable Rust program, and (3) Enhance the correctness of the translated Rust program by using test cases to check input/output equivalence, isolate faulty code when execution states deviate, and iteratively refine the translation using feedback from compilation and test errors. We empirically evaluate RustMap on 126 real-world programs, including 125 from Rosetta Code and a 7000+ line bzip2 implementation using GPT-4o as the LLM. RustMap shows promising results, guiding GPT-4o to produce idiomatic, readable, and functional Rust code with significantly less unsafe code than other tools, and revealing non-trivial translation patterns reusable for future research.

==> sections/challenges.tex <==


In the realm of translating existing C to Rust, C2Rust is the state-of-the-art automation tool that translates most C modules into semantically equivalent Rust code. These modules are intended to be compiled in isolation to produce compatible object files. In the process of translating C code to Rust, C2Rust researchers encounter multiple challenges \cite{c2rust_challenges}:
\textbf{Firstly}, the issue of build system integration involves handling and translating the compilation commands and dependencies involved in a project's build process, as addressed in Section \ref{sec:project-scale-synthesis}. \textbf{Secondly}, the use of the C Preprocessor (\texttt{cpp}) adds complexity because it operates at the level of string concatenation without adhering to C's syntactic structures. This is discussed in \ref{empirical-numerical-macro} and \ref{empirical-complex-macro}. \textbf{Thirdly}, Rust does not support \texttt{goto} statements or fall-through in \texttt{switch} statements, necessitating detailed control flow adjustments during translation, as detailed in \ref{sec-switch-case-rewrite-rust}. \textbf{Additionally}, Rust's stringent static variable initialization, handling of Variable Length Arrays (VLA) via the Vec type, and limited but workable support for variadic functions through C function imports, underscore the translation challenges we plan to tackle in future work.

Given the huge demand for rewriting C/C++ projects to Rust, we need to address several questions:
C2Rust, despite its capabilities, faces several limitations when translating C code to Rust:
\textbf{Limitations of C2Rust in Handling Project-Level C}
C2Rust, despite its capabilities, faces several significant limitations when translating C code to Rust:

Firstly, handling large projects is a significant challenge. After preprocessing, C2Rust merges all \texttt{*.c} and \texttt{*.h} files into \texttt{*.i} files and then generates a single \texttt{*.rs} file. This approach lacks separation and specialization, resulting in a large, complex code structure that is hard to manage and maintain. Additionally, developers often cannot directly use C2Rust to compile Rust code as it does not always generate \texttt{Cargo.toml} or \texttt{build.rs} to build the project. There may also be many C libraries incompatible with the current Rust release, and there are no additional functional tests on the generated Rust project. \label{paragraph:large-projects}

Secondly, dealing with C macros presents issues. C2Rust expands all macros during preprocessing, directly incorporating these expansions into the translated code. This often leads to code bloat and a loss of macro functionality, making the translated code less maintainable. Furthermore, understanding function relationships is another challenge not explicitly addressed by C2Rust. The tool operates without human intervention and does not consider how functions call each other, which can result in poorly structured and inefficient code translation. \label{paragraph:c-macros}

Moreover, at the function level, C2Rust converts code directly based on the abstract syntax tree (AST), frequently introducing a significant amount of unsafe code, which contradicts Rust's safety guarantees and best practices. When it comes to smaller code fragments, including complex control flows and pointer management, C2Rust handles the conversion in a less systematic manner. This can lead to inaccuracies and difficulties in maintaining the translated code. \label{paragraph:function-level}

Finally, C2Rust lacks a robust process for continuous improvement. There is no built-in mechanism for ongoing testing and optimization to meet performance and reliability standards. Additionally, rewriting C to Rust without knowing the design rationale can be challenging. Despite the significant demand in the industry for enhanced safety, performance, and maintainability that Rust offers, many organizations face difficulties in rewriting or upgrading key software components. This challenge is compounded by the lack of comprehensive documentation or the original developers' inputs. \label{paragraph:continuous-improvement}


==> sections/complexmacro.tex <==


% \lx{Also, would be good to have an example how a complex macro involving control-flow changes is translated; or add a goto example in Section~\ref{sec:goto}, and just refer to that.}
In the C code (Figure \ref{lst:complex_macro_definition_C}), the macro \texttt{GET\_BITS} is used to handle bitstream manipulation. The macro is defined with multiple lines and includes a \texttt{return} statement, making it complex and harder to maintain.
As we mentioned in \ref{sec:fn-depencies-synthesis}, we converted the complex macros in C into functions to ensure that they appear in the call graph of the *.i files instead of being replaced by text.
To address this complexity, we have rewritten the macro as two separate functions in Rust (Figure \ref{lst:complex_macro_definition_rewrite_rust}). This separation improves readability and maintainability by handling the return logic and bitstream manipulation separately.

% \new{
Complex macros are processed by converting them into functions before generating the call graph. This conversion facilitates improved readability and clearer control-flow relationships after the transition to Rust.

\begin{figure}[h]
\centering
    % \inputminted[frame=single, fontsize=\scriptsize]{c}{COMPLEXMACROS/Complex_Def_C_macro.c}
\begin{minted}[frame=single, fontsize=\scriptsize]{c}
// decompress.c
#define RETURN(rrr)                               \
   { retVal = rrr; goto save_state_and_return; };


#define GET_BITS(lll,vvv,nnn)
   while (True) {
      if (s->bsLive >= nnn) {                     
         UInt32 v;
         v = (s->bsBuff >>
             (s->bsLive-nnn)) & ((1 << nnn)-1);
         s->bsLive -= nnn;
         vvv = v;
         break;
      }                                    
      if (s->strm->avail_in == 0) RETURN(BZ_OK);
      s->bsBuff
         = (s->bsBuff << 8) |
           ((UInt32)
              (*((UChar*)(s->strm->next_in))));
      s->bsLive += 8;
      s->strm->next_in++;
      s->strm->avail_in--;
      s->strm->total_in_lo32++;
      if (s->strm->total_in_lo32 == 0)
         s->strm->total_in_hi32++;
   }
}
\end{minted}
\caption{Original Definition of Complex Macro in C}
\label{lst:complex_macro_definition_C}
\end{figure}

\begin{figure}[h]
\centering
    % {COMPLEXMACROS/Complex_Def_C_fn.c}
\begin{minted}[frame=single, fontsize=\scriptsize]{c}
int GET_BITS_first_half(DState *s, uint32_t *vvv, int nnn) {
    if (s->bsLive >= nnn) {
        uint32_t v = (s->bsBuff >> (s->bsLive - nnn)) & ((1u << nnn) - 1);
        s->bsLive -= nnn;
        *vvv = v;

        // Debug output, always printed if this function is called
        printf("vvv: %u\n", *vvv);
        return 1; // OK
    } else {
        return 0; // ERROR
    }
}

void GET_BITS_second_half(DState *s) {
    s->bsBuff = (s->bsBuff << 8) | 
    *((uint8_t*)(s->strmD->next_in_pointer));
    s->bsLive += 8;
    s->strmD->next_in_pointer++; 
    s->strmD->avail_in--;
    s->strmD->total_in_lo32++;
    if (s->strmD->total_in_lo32 == 0) {
        s->strmD->total_in_hi32++;
    }
}
\end{minted}
\caption{Rewrite Definition of Complex Macro Rewrite as C Function}
\label{lst:complex_macro_definition_rewrite_rust}
\end{figure}

The examples in Figures \ref{lst:complex_macro_definition_C} and \ref{lst:complex_macro_definition_rewrite_rust} illustrate how the \texttt{GET\_BITS} macro, used in the \texttt{decompress} function, is refactored into Rust functions. This approach retains control flow, particularly the exit points, ensuring the translated Rust code is both clear and maintainable.




==> sections/fail.tex <==
\jk{todo: add the examples that are failed across tools}

==> sections/preprocessing.tex <==

\subsection{Macro Translation}
\label{sec:macros}


==> sections/rustmap.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{pic/rustmap-overview-diagram.png}
    \caption{RustMap Approach Overview}
    \label{fig:rustmap-overview}
\end{figure}
RustMap aims to convert entire C  to Rust at the project level.The conversion process follows a systematic approach as illustrated in the overview diagram in \textbf{Methodology}:
\begin{enumerate}
    \item \textbf{Project-Scale Scaffolding}: Our approach sets up the foundational structure of the project by generating \texttt{scc\_number\_function\_name.rs} files, creating a more modular and maintainable codebase, clearly mapping dependencies and interactions. This addresses the issues described in \ref{paragraph:large-projects} and \ref{paragraph:build-issues} (see details in Section \ref{sec:project-scale-synthesis}).

    \item \textbf{C Macros Refactoring}: We retain the macro abstraction where possible, translating macros in a way that preserves their original intent and utility in the Rust codebase. This improves maintainability and functionality, tackling the problems highlighted in \ref{paragraph:c-macros} and \ref{paragraph:function-relationships} (see details in Section \ref{sec:macro-refactoring}).

    \item \textbf{Function-Dependencies Synthesis}: By understanding function call relationships, we systematically number functions based on their dependencies, guiding the translation process in a structured manner. This interactive process ensures dependencies are resolved correctly and efficiently, reducing translation errors, as noted in \ref{paragraph:function-level} (see details in Section \ref{sec:fn-depencies-synthesis}).

    \item \textbf{Function-Level Synthesis}: We emphasize idiomatic safe Rust, implementing a step-by-step process for each Translation Unit or Function SCC. This method involves testing and compiling in small increments, using Delta-Debugging and bug localization techniques to pinpoint errors, as discussed in \ref{paragraph:function-level} and \ref{paragraph:continuous-improvement} (see details in Section \ref{sec:fn-level-synthesis}).

    \item \textbf{Code-Fragment-Level Synthesis}: This step handles the conversion of smaller code fragments, including complex control flows and pointer management, in a systematic manner, ensuring accuracy and safety in the translated Rust code, as mentioned in \ref{paragraph:function-level} (see details in Section \ref{sec:code-fragment-synthesis}).

    \item \textbf{Iterative Refinement}: The process concludes with continuous testing and optimization to meet performance and reliability standards. This involves iterative testing, feedback incorporation, and code refinement, addressing the needs described in \ref{paragraph:continuous-improvement}.
\end{enumerate}


\textbf{Empirical Study}: Throughout the synthesis processes, continuous evaluation and iteration ensure the translated Rust code is functionally equivalent to the original C code while leveraging Rust's safety and performance features. The study includes a Translation Result Summary, highlighting successful implementation and improvements in safety metrics compared to C2Rust (see details in Section \ref{sec:trans-result-summary}). Translation Cases Study provides detailed examples of the refactoring and synthesis processes (see details in Section \ref{sec:trans-case-study}). Lastly, a Coverage Test demonstrates how extensively the translated Rust code covers the functionality of the original C code (see details in Section \ref{sec:trans-coverage-test}).

This section provides a comprehensive overview of the methodology employed in converting a C project to Rust. It details the project-scale scaffolding techniques, including how to structure the Rust project using cargo, and explains the handling of headers and global files. The process of rewriting global variables using lazy\_static for thread safety is covered. Furthermore, it delves into macro refactoring and the generation of function call graphs to understand function dependencies. The section concludes with strategies for translating functions from C to Rust using delta-debugging techniques to ensure accuracy and consistency.

\subsection{Challenges and Questions of C2Rust}
\label{challenges-questions-c2rust}
\input{sections/challenges.tex}


